MGQL: An Executable, Small-Step Semantics of GQL

ISO Graph Query Language (GQL) is the first international standard for property graph-based graph query languages, standardized as ISO/IEC 39075 in 2024. However, ISO/IEC 39075 codifies its semantics informally across 600+ pages of prose, making it difficult to formally reason about the standard or for a standard-faithful implementation. Existing formalizations are not adequate because they either: (1) significantly reduce the semantic complexity by omitting bag semantics, schemas, and composite queries on multiple graphs; (2) or significantly reduce the syntactic complexity by only considering isolated fragments such as pattern-matching, leaving the full query pipeline unformalized. Yet it is these semantic-syntactic features that make formalizing GQL non-trivial. We present MGQL, the first mechanized, small-step operational semantics for a substantial read-only fragment of GQL that is grounded in the ISO/IEC 39075 standard. Our formalization models multi-graph property graphs with mixed edge directionality and supports a large fraction of GQL pattern constructs: quantified paths and edges, directional and undirected matching, label expressions, pattern lists, and composite queries. The semantics is supported by a schema-aware type system that refines variable types via closed-graph schemas, tracks nullability, supports multiple composite query operators, and models quantified-path bindings with list types. We prove that our type system is sound, ensuring an end-to-end guarantee of well-formed queries yielding results that conform to their declared schemas. MGQL provides the first bridge between GQL's informal specification and a mechanized implementation, enabling formal reasoning about correctness.

==> figures/property-graph-querying-tikz.tex <==
\begin{tikzpicture}[
  font=\footnotesize,
  >=Latex,
  node distance=15mm and 20mm,
  vertex/.style={
    circle,
    draw,
    thick,
    white,
    minimum size=6mm,
    inner sep=0pt,
    draw opacity=0.35,
    fill opacity=0.35,
    text opacity=0.35,
    align=center
  },
  vertexMatch/.style={
    circle,
    draw,
    thick,
    white,
    minimum size=6mm,
    inner sep=0pt,
    align=center
  },
  numberMatch/.style={
    circle,
    draw=purple!90!black,
    fill=white,
    text=purple!90!black,
    thick,
    font=\bfseries\small,
    minimum size=3.2mm,
    inner sep=0pt,
    align=center
  },
  person/.style={vertex, fill=blue!20},
  personMatch/.style={vertexMatch, fill=blue!20},
  pattern/.style={numberMatch},
  company/.style={vertex, fill=orange!20},
  proj/.style={vertex, fill=purple!20},
  projMatch/.style={vertexMatch, fill=purple!20},
  vname/.style={font=\bfseries, text opacity=0.35},
  vnameMatch/.style={font=\bfseries},
  vlabel/.style={font=\scriptsize, yshift=-5mm, text opacity=0.35},
  callout/.style={
    draw=black!80,
    rounded corners=1pt,
    %thin,
    fill=black!6,
    font=\scriptsize,
    inner sep=2pt,
    align=left
  },
  rel/.style={
    -{Latex[length=2mm,width=1.6mm]},
    thin,
    draw=black!55
  },
  relMatch/.style={
    -{Latex[length=2mm,width=1.6mm]},
    thick,
    draw=purple!90!black
  },
  rlabel/.style={
    fill=white,
    inner sep=1.2pt,
    font=\scriptsize,
    text opacity=0.55
  },
  rlabelMatch/.style={
    fill=white,
    inner sep=1.2pt,
    font=\scriptsize
  },
  frame/.style={draw, rounded corners=3pt, thin, inner sep=7pt}
]

% Persons
\node[personMatch] (a) at (0.5,0) {};
\node[vnameMatch] at (a) {a};
\node[vlabel] at (a) {};

\node[pattern, above=1pt] at (a.north) {1};
\node[pattern, below right=1mm and 0.5pt of a] at (a.east) {2};

\node[personMatch] (b) at (2,1.4) {};
\node[vnameMatch] at (b) {b};
\node[vlabel] at (b) {};

\node[personMatch] (c) at (2,-1.4) {};
\node[vnameMatch] at (c) {c};
\node[vlabel] at (c) {};

\node[pattern, above right=1pt and 4pt of c] at (c.north) {3};

\node[person] (d) at (3.5,0.0) {};
\node[vname] at (d) {d};
\node[vlabel] at (d) {};

\node[person] (e) at (4,-2.0) {};
\node[vname] at (e) {e};
\node[vlabel] at (e) {};

% Companies
\node[company] (x) at (0,-2.0) {};
\node[vname] at (x) {x};
\node[vlabel] at (x) {};

\node[company] (y) at (4,2.0) {};
\node[vname] at (y) {y};
\node[vlabel] at (y) {};

% Project
\node[projMatch] (p) at (0,2.0) {};
\node[vnameMatch] at (p) {p};
\node[vlabel] at (p) {};

% Node types
\node[vlabel] (spacing) at (0,-2.9) {};
\node[personMatch] (f) at (0,-3.8) {};
\node[vnameMatch] at (f) {a};
\node[personMatch] (z) at (2,-3.8) {};
\node[vnameMatch] at (z) {a};
\node[personMatch] (q) at (4,-3.8) {};
\node[vnameMatch] at (q) {c};
\node[
  draw,
  thick,
  rectangle,
  rounded corners=1pt,
  fit=(spacing)(f)(z)(q),
  inner sep=2pt,
] (infoBox) {};

\node[
  draw,
  thick,
  rounded corners=0.5pt,
  fill=white,
  inner sep=2pt,
] at (infoBox.north) {\small $\fReturn$ \textcolor{purple!90!black}{\fCyNode{m}}; \textbf{(Bag Semantics)}};


% KNOWS edges
\draw[relMatch] (a) to[bend left=12] node[rlabelMatch, midway] {\texttt{KNOWS}} (b);
\draw[rel] (b) to[bend left=12] node[rlabel, midway] {\texttt{KNOWS}} (d);
\draw[relMatch] (a) to[bend right=12] node[rlabelMatch, midway] {\texttt{KNOWS}} (c);
\draw[rel] (c) to[bend right=14] node[rlabel, midway] {\texttt{KNOWS}} (d);
\draw[relMatch] (c) -- node[rlabelMatch, midway] {\texttt{KNOWS}} (b);
\draw[rel] (c) to[bend right=12] node[rlabel, midway] {\texttt{KNOWS}} (e);
\draw[rel] (d) to[bend left=12] node[rlabel, midway] {\texttt{KNOWS}} (e);

% WORKS edges
\draw[rel] (a) to[bend right=12] node[rlabel, midway, yshift=2pt] {\texttt{WORKS}} (x);
\draw[rel] (c) to[bend left=14] node[rlabel, midway, xshift=4pt, yshift=1pt] {\texttt{WORKS}} (x);
\draw[rel] (b) -- node[rlabel, midway, xshift=-4pt, yshift=-1pt] {\texttt{WORKS}} (y);
\draw[rel] (d)  to[bend right=14] node[rlabel, midway, xshift=-1pt, yshift=-4pt] {\texttt{WORKS}} (y);

\draw[relMatch] (b) -- node[rlabelMatch, midway, xshift=3pt, yshift=-1pt] {\texttt{LEADS}} (p);

% FUNDS edges
\draw[rel] (y) to[bend right=20] node[rlabel, midway] {\texttt{FUNDS}} (p);
\draw[rel] (x) to[bend left=20] node[rlabel, midway] {\texttt{FUNDS}} (p);

% INVESTS edges
\draw[rel] (e) to[bend right=20] node[rlabel, midway] {\texttt{INVESTS}} (y);
\draw[rel] (e) to[bend left=20] node[rlabel, midway] {\texttt{INVESTS}} (x);
\end{tikzpicture}


==> figures/propgraph-gql-example.tex <==
\begin{figure}[t]%
  \centering%
  \begin{subfigure}[b]{0.46\linewidth}%
    \centering%
    \resizebox{1.0\linewidth}{!}{\input{figures/property-graph-tikz}}%
    \vspace{-1mm}%
    \caption{\FigCaptionPropGraphInstance}%
    %\vspace{2mm}%
  \end{subfigure}%
  \hfill
  \begin{subfigure}[b]{0.52\linewidth}%
    \centering%
    \hspace*{7mm}%
    \begin{minipage}{1.0\linewidth}%
\begin{CypherBox}        
(*@$\fMatch\;\;$@*)(*@{$\textcolor{\ExamplePatMatchNodeColor}{\fCyElemNodePattern{\fCyNode{m}}}\textcolor{\ExamplePatKnowsEdgeColor}{\fCyEdgeRight{\fCyElemEdgePattern{\text{\texttt{\!:KNOWS}}}}\!\fCyQuantBound{1}{2}}\,\textcolor{\ExamplePatPersonNodeColor}{\fCyElemNodePattern{\phantom{i}}}\textcolor{\ExamplePatLeadsEdgeColor}{\fCyEdgeRight{\fCyElemEdgePattern{\text{\texttt{\!:LEADS}}}}}\,\textcolor{\ExamplePatProjectNodeColor}{\fCyElemNodePattern{\phantom{i}}}$}@*)
\end{CypherBox}%
    \end{minipage}%
    \vspace{3mm}%
    \\
    \begin{minipage}{1.0\linewidth}%
    \resizebox{0.9\linewidth}{!}{\input{figures/property-graph-querying-tikz-1}}%
    \end{minipage}%
    \vspace{-1mm}%
    \hspace*{-6mm}%
    \caption{\FigCaptionGqlExample}%
    %\vspace{2mm}%
  \end{subfigure}%
  \vspace{2mm}%
  \\
  \begin{subfigure}[b]{1.0\linewidth}%
    \centering%
    \begin{GrammarBox}%
      \begin{minipage}{0.95\linewidth}%
        \input{formalizations/gql-calculus}%
      \end{minipage}%
    \end{GrammarBox}%
    \vspace{-3mm}%
    \caption{\FigCaptionGqlCalculus}%
    %\vspace{4mm}%
  \end{subfigure}%
  \vspace{-1mm}%
  \caption{\FigCaptionPropertyGraphsAndGql}%
\end{figure}%


==> formalizations/gql-node.tex <==
\begin{mathpar}
    %\mprset{vskip=1mm}
    \infer[\RuleNameFont\FTySAtomLabelPropFresh]
    {
      \fVar{\fCyPatternAtom} \in \fAttr\\
      \fPropJudge{}{\fProp{\fCyPatternAtom}}{\fDbPropSchema}\\
      %% \fPropJudge{\fDbWorld;\varnothing}
      %%            {\fPGProp}
      %%            {\fDbPropSchema[\fPGProp]}\\
      \fLabelSJudge{\fDbElemSchema}{\fLbl{\fCyPatternAtom}}{\fDbElemSchema[\textsf{l}]}\\
      \fPropSJudge{\fDbElemSchema}{\fDbPropSchema}{\fDbElemSchema[\fDbPropSchema]}
    }
    {
      \fSAtomJudge{\fDbElemSchema}
                 {\fCyPatternAtom}
                 {\fDbElemSchema[\textsf{l}]\cap\fDbElemSchema[\fDbPropSchema]}
    }
%    \and
    %% \infer[\RuleNameFont\FTySNodeLabelProp]
    %% {
    %%   \fCyNodeVar \in \fDom{\fDbRSchema}\quad
    %%   \fDbNodeType[{\fDbGNames,\fDbNodeSchema[\fCyNodeVar]}]?=\fDbRSchema(\fCyNodeVar)\quad
    %%   \fPropJudge{\fDbWorld;\fDbRSchema}
    %%              {\fPGProp}
    %%              {\fDbPropSchema[\fPGProp]}\\\\
    %%   \fDbGNames \in \fDom{\fDbSchema}\quad
    %%   \fDbGraphSchema=\fDbSchema(\fDbGNames)\quad
    %%   \fLabelSJudge{\fDbGraphSchema}{\fPGNodelabel}{\fDbNodeSchema[l]}\quad
    %%   \fPropSJudge{\fDbGraphSchema}{\fDbPropSchema[\fPGProp]}{\fDbNodeSchema[\fPGProp]}
    %% }
    %% {
    %%   \fSNodeJudge{\fDbWorld;\fDbRSchema}
    %%              {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel\,\fPGProp}\;}
    %%              {\fDbNodeSchema[l]\cap\fDbNodeSchema[\fPGProp]\cap\fDbNodeSchema[\fCyNodeVar]}
    %% }
    %% \and
    %% \infer[\RuleNameFont\FTySNodeLabelPropNull]
    %% {
    %%   \fCyNodeVar \in \fDom{\fDbRSchema}\\
    %%   ?\fDbNodeType=\fDbRSchema(\fCyNodeVar)\\
    %%   \fDbGNames \in \fDom{\fDbSchema}
    %% }
    %% {
    %%   \fSNodeJudge{\fDbWorld;\fDbRSchema}
    %%              {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel\,\fPGProp}\;}
    %%              {\varnothing}
    %% }
    %% \and
    %% \infer[\RuleNameFont\FTySEdgeLabelPropNull]
    %% {
    %%   \fCyEdgeVar \in \fDom{\fDbRSchema}\\
    %%   ?\fDbEdgeType=\fDbRSchema(\fCyEdgeVar)\\
    %%   \fDbGNames \in \fDom{\fDbSchema}
    %% }
    %% {
    %%   \fSEdgeJudge{\fDbWorld;\fDbRSchema}
    %%              {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel\,\fPGProp}\;}
    %%              {\varnothing}
    %% }
    %% \and
    %% \infer[\RuleNameFont\FTySEdgeLabelPropFresh]
    %% {
    %%   \fVar{\fCyPatternEdge} \in \fAttr\quad\;
    %%   \fDbGNames \in \fDom{\fDbSchema}\quad\;
    %%   \fPropJudge{}{\fProp{\fCyPatternEdge}}{\fDbPropSchema}\\\\
    %%   (-,\fDbEdgeSchema)=\fDbSchema(\fDbGNames)\quad\;
    %%   %% \fPropJudge{\fDbWorld;\varnothing}
    %%   %%            {\fPGProp}
    %%   %%            {\fDbPropSchema[\fPGProp]}\\
    %%   \fLabelSJudge{\fDbEdgeSchema}{\fLbl{\fCyPatternEdge}}{\fDbEdgeSchema[\textsf{l}]}\quad\;
    %%   \fPropSJudge{\fDbEdgeSchema}{\fDbPropSchema}{\fDbEdgeSchema[\textsf{p}]}
    %% }
    %% {
    %%   \fSEdgeJudge{\fDbWorld}
    %%              {\fCyPatternEdge}
    %%              {\fDbEdgeSchema[\textsf{l}]\cap\fDbEdgeSchema[\textsf{p}]}
    %% }
    %% \and
    %% \infer[\RuleNameFont\FTySEdgeLabelProp]
    %% {
    %%   \fCyEdgeVar \in \fDom{\fDbRSchema}\quad
    %%   \fDbEdgeType[{\fDbGNames,\fDbEdgeSchema[\fCyEdgeVar]}]?=\fDbRSchema(\fCyEdgeVar)\quad
    %%   \fPropJudge{\fDbWorld;\fDbRSchema}
    %%              {\fPGProp}
    %%              {\fDbPropSchema[\fPGProp]}\\\\
    %%   \fDbGNames \in \fDom{\fDbSchema}\quad
    %%   \fDbGraphSchema=\fDbSchema(\fDbGNames)\quad
    %%   \fLabelSJudge{\fDbGraphSchema}{\fPGNodelabel}{\fDbEdgeSchema[l]}\quad
    %%   \fPropSJudge{\fDbGraphSchema}{\fDbPropSchema[\fPGProp]}{\fDbEdgeSchema[\fPGProp]}
    %% }
    %% {
    %%   \fSEdgeJudge{\fDbWorld;\fDbRSchema}
    %%              {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel\,\fPGProp}\;}
    %%              {\fDbEdgeSchema[l]\cap\fDbEdgeSchema[\fPGProp]\cap\fDbEdgeSchema[\fCyEdgeVar]}
    %% }
    %% \and
    %% \infer[\RuleNameFont\FTySNodeLabel]
    %% {
    %%   \fSNodeJudge{\fDbWorld;\fDbRSchema}
    %%               {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodeLabel\,\varnothing}\;}
    %%               {(\fPGNodeLabel,\varnothing)}
    %% }
    %% {
    %%   \fSNodeJudge{\fDbWorld;\fDbRSchema}
    %%              {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodeLabel}\;}
    %%              {(\fPGNodeLabel,\varnothing)}
    %% }
    %% \and
    %% \infer[\RuleNameFont\FTySNodeProp]
    %% {
    %%   \fSNodeJudge{\fDbWorld;\fDbRSchema}
    %%               {\fCyElemNodePattern{\fCyNodeVar\,\varnothing\,\fPGProp}\;}
    %%              {(\varnothing,\fDbPropSchema[\fPGProp])}
    %% }
    %% {
    %%   \fSNodeJudge{\fDbWorld;\fDbRSchema}
    %%              {\fCyElemNodePattern{\fCyNodeVar\,\fPGProp}\;}
    %%              {(\varnothing,\fDbPropSchema[\fPGProp])}
    %% }
  %%%%%%% Patterns %%%%%%%%%
  %% \infer[\RuleNameFont\FTyPNodeAtom]
  %%   {
  %%     \fSNodeJudge{\fDbWorld;\fDbRSchema}
  %%                {\fCyElemNodePattern{\fCyNodeVar}\;}
  %%                {(\varnothing,\varnothing)}
  %%   }
  %%   {
  %%     \fNodeJudge{\fDbWorld;\fDbRSchema}
  %%                {\fCyElemNodePattern{\fCyNodeVar}}
  %%                {\fDbRSchema[\fCyNodeVar \mapsto \fDbNodeType]} 
  %%   }
  %%   \and
  %%   \infer[\RuleNameFont\FTyPNodeLabel]
  %%   {
  %%     \fSNodeJudge{\fDbWorld;\fDbRSchema}
  %%                {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodeLabel\,\varnothing}\;}
  %%                {(\fPGNodeLabel,\varnothing)} 
  %%   }
  %%   {
  %%     \fPatJudge{\fDbWorld;\fDbRSchema}
  %%                {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodeLabel}}
  %%                {\fDbRSchema[\fCyNodeVar \mapsto \fDbNodeType]} 
  %%   }
  %%   \and
  %%   \infer[\RuleNameFont\FTyPNodeProp]
  %%   {
  %%     \fSNodeJudge{\fDbWorld;\fDbRSchema}
  %%                {\fCyElemNodePattern{\fCyNodeVar\,\varnothing\,\fPGProp}\;}
  %%                {(\varnothing,\fDbPropSchema[\fPGProp])} 
  %%   }
  %%   {
  %%     \fPatJudge{\fDbWorld;\fDbRSchema}
  %%                {\fCyElemNodePattern{\fCyNodeVar\,\fPGProp}}
  %%                {\fDbRSchema[\fCyNodeVar \mapsto \fDbNodeType]} 
  %%   }
  %%   \and
\end{mathpar}


==> formalizations/gql-pattern-atom-anon.tex <==
\begin{mathpar}
    \infer[\RuleNameFont\FRenNode]
    {
      \phantom{a}        
    }
    {
      \fAnonJudge{\fDbVarUse}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fCyLabelExp\,\fPGProp}}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fCyLabelExp\,\fPGProp}}
                 {\fDbVarUse\cup\fSet{\fCyNodeVar}}
    }
    \and
    \infer[\RuleNameFont\FRenEdge]
    {
      \phantom{a}       
    }
    {
      \fAnonJudge{\fDbVarUse}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel\,\fPGProp\,\fCyDir}}
                 {\fCyElemNodePattern{\varepsilon\,\varepsilon\,\varnothing}\,\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel\,\fPGProp\,\fCyDir}\,\fCyElemNodePattern{\varepsilon\,\varepsilon\,\varnothing}}
                 {\fDbVarUse\cup\fSet{\fCyEdgeVar}}
    }
    \\
    \infer[\RuleNameFont\FRenNodeB]
    {
      \fCyNodeVar\in\fAttrAnon\setminus\fDbVarUse        
    }
    {
      \fAnonJudge{\fDbVarUse}
                 {\fCyElemNodePattern{\varepsilon\,\fCyLabelExp\,\fPGProp}}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fCyLabelExp\,\fPGProp}}
                 {\fDbVarUse\cup\fSet{\fCyNodeVar}}
    }
    \and
    \infer[\RuleNameFont\FRenEdgeB]
    {
      \fCyEdgeVar\in\fAttrAnon\setminus\fDbVarUse
    }
    {
      \fAnonJudge{\fDbVarUse}
                 {\fCyElemEdgePattern{\varepsilon\,\fPGNodelabel\,\fPGProp\,\fCyDir}}
                 {\fCyElemNodePattern{\varepsilon\,\varepsilon\,\varnothing}\,\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel\,\fPGProp\,\fCyDir}\,\fCyElemNodePattern{\varepsilon\,\varepsilon\,\varnothing}}
                 {\fDbVarUse\cup\fSet{\fCyEdgeVar}}
    }
\end{mathpar}


==> formalizations/gql-pattern-quantified-typing.tex <==
\begin{mathpar}

\end{mathpar}


==> formalizations/gql-pattern-typing-forward-closed.tex <==
\begin{mathpar}
    \infer[\RuleNameFont\FTyPPatLabelPropClosedSrc]
    {
      \fDbGNames \in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      \fPatJudge{\fDbWorld;\fDbRSchemas{2}}
                {\fCyNodeVar,\,\fCyEdgeVar}
                {\fDbRSchemas{3}}
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}
                   \fCyEdgeRight{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 }
                 {\fDbRSchemas{3}}
    }
    \quad
    \infer[\RuleNameFont\FTyPPatLabelPropClosedDst]
    {
      \fDbGNames \in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      \fPatJudge{\fDbWorld;\fDbRSchemas{2}}
                {\fCyEdgeVar,\,\fCyNodeVar}
                {\fDbRSchemas{3}}
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[2]\,\fPGProp[2]}
                   \fCyEdgeLeft{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 }
                 {\fDbRSchemas{3}}
    }
    \and
    \infer[\RuleNameFont\FTyPPatLabelPropClosedSrcFail]
    {
      \fDbGNames \in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      ?\fDbNodeType = \fDbRSchemas{2}(\fCyNodeVar)\;\lor\;
      ?\fDbEdgeType = \fDbRSchemas{2}(\fCyEdgeVar)
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}
                   \fCyEdgeRight{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 }
                 {\fDbRSchemas{2}[
                     \fCyNodeVar \mapsto ?\fDbNodeType,
                     \fCyEdgeVar \mapsto ?\fDbEdgeType
                 ]}
    }
    \quad
    \infer[\RuleNameFont\FTyPPatLabelPropClosedDstFail]
    {
      \fDbGNames \in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      ?\fDbEdgeType = \fDbRSchemas{2}(\fCyEdgeVar)\;\lor\;
      ?\fDbNodeType = \fDbRSchemas{2}(\fCyNodeVar)
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[2]\,\fPGProp[2]}
                   \fCyEdgeLeft{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 }
                 {\fDbRSchemas{2}[
                     \fCyEdgeVar \mapsto ?\fDbEdgeType,
                     \fCyNodeVar \mapsto ?\fDbNodeType
                 ]}
    }
    \and
    \infer[\RuleNameFont\FTyPPatList]
    {
      \fCyPatterns=\fConcat{\fCyPatterns'}{\fCyPattern}\\      
      \fPatJudge{\fDbWorld;\fDbRSchema}{\fCyPatterns'}{\fDbRSchemas{1}}\\
      \fPatJudge{\fDbWorld;\fDbRSchema}{\fCyPattern}{\fDbRSchemas{2}}\\
      \mathcal{D}=\fDom{\fDbRSchemas{1}}\cap\fDom{\fDbRSchemas{2}}\\
      \fCompatSub{\fDbRSchemas{1}}{\fDbRSchemas{2}}{\mathcal{D}}\;\lor\;
      \mathcal{D}=\varnothing
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                {\fCyPatterns}
                {\fSchemaJoin{\fDbRSchemas{1}}{\fDbRSchemas{2}}}
    }
\end{mathpar}


==> formalizations/gql-pattern-typing-forward-open.tex <==
\begin{mathpar}
    \infer[\RuleNameFont\FTyPNodeLabelPropOpen]
    {
      \fDbGNames \not\in \fDom{\fDbSchema}\\
      \fCyNodeVar \not\in \fDom{\fDbRSchema}\\
      \fCyNodeVar \in \fAttr
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel\,\fPGProp}}
                 {\fDbRSchema[\fCyNodeVar \mapsto \fDbNodeType?]} 
    }
    %% \and
    %% \infer[\RuleNameFont\FTyPNodeLabelPropOpenBound]
    %% {
    %%   \fDbGNames \not\in \fDom{\fDbSchema}\\
    %%   \fCyNodeVar \in \fDom{\fDbRSchema}\\
    %%   \fDbNodeType?=\fDbRSchema(\fCyNodeVar)\;\lor\;
    %%   ?\fDbNodeType=\fDbRSchema(\fCyNodeVar)
    %% }
    %% {
    %%   \fPatJudge{\fDbWorld;\fDbRSchema}
    %%              {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel\,\fPGProp}}
    %%              {\fDbRSchema} 
    %% }
    \and
    \infer[\RuleNameFont\FTyPEdgeLabelPropOpen]
    {
      \fDbGNames \not\in \fDom{\fDbSchema}\\
      \fCyEdgeVar \not\in \fDom{\fDbRSchema}\\ 
      \fCyEdgeVar \in \fAttr
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel\,\fPGProp}}
                 {\fDbRSchema[\fCyEdgeVar \mapsto \fDbEdgeType?]} 
    }
    %% \and
    %% \infer[\RuleNameFont\FTyPEdgeLabelPropOpenBound]
    %% {
    %%   \fDbGNames \not\in \fDom{\fDbSchema}\\
    %%   \fCyEdgeVar \in \fDom{\fDbRSchema}\\
    %%   \fDbEdgeType?=\fDbRSchema(\fCyEdgeVar)\;\lor\;
    %%   ?\fDbEdgeType=\fDbRSchema(\fCyEdgeVar)
    %% }
    %% {
    %%   \fPatJudge{\fDbWorld;\fDbRSchema}
    %%              {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel\,\fPGProp}}
    %%              {\fDbRSchema} 
    %% }
    \and
    \infer[\RuleNameFont\FTyPPatLabelPropOpenSrc]
    {
      \fDbGNames \not\in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      ?\fDbNodeType \neq \fDbRSchemas{2}(\fCyNodeVar)\\
      ?\fDbEdgeType \neq \fDbRSchemas{2}(\fCyEdgeVar)
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}
                   \fCyEdgeRight{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 }
                 {\fDbRSchemas{2}}
    }
    \quad
    \infer[\RuleNameFont\FTyPPatLabelPropOpenDst]
    {
      \fDbGNames \not\in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      ?\fDbEdgeType \neq \fDbRSchemas{2}(\fCyEdgeVar)\\
      ?\fDbNodeType \neq \fDbRSchemas{2}(\fCyNodeVar)
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyEdgeRight{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[2]\,\fPGProp[2]}
                 }
                 {\fDbRSchemas{2}}
    }
    \and
    \infer[\RuleNameFont\FTyPPatLabelPropOpenSrcNull]
    {
      \fDbGNames \not\in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      ?\fDbNodeType = \fDbRSchemas{2}(\fCyNodeVar)\;\lor\;
      ?\fDbEdgeType = \fDbRSchemas{2}(\fCyEdgeVar)
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}
                   \fCyEdgeRight{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 }
                 {\fDbRSchemas{2}[
                     \fCyNodeVar \mapsto ?\fDbNodeType,
                     \fCyEdgeVar \mapsto ?\fDbEdgeType
                 ]}
    }
    \quad
    \infer[\RuleNameFont\FTyPPatLabelPropOpenDstNull]
    {
      \fDbGNames \not\in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      ?\fDbEdgeType = \fDbRSchemas{2}(\fCyEdgeVar)\;\lor\;
      ?\fDbNodeType = \fDbRSchemas{2}(\fCyNodeVar)
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyEdgeRight{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[2]\,\fPGProp[2]}
                 }
                 {\fDbRSchemas{2}[
                     \fCyEdgeVar \mapsto ?\fDbEdgeType,
                     \fCyNodeVar \mapsto ?\fDbNodeType
                 ]}
    }
\end{mathpar}


==> formalizations/gql-pattern-typing-undirected.tex <==
\begin{mathpar}
    \infer[\RuleNameFont\FTyPPatClosedUDir]
    {
      \fDbGNames \in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      \fDbNodeType[{\fDbGNames,\fDbNodeSchema}]?=\fDbRSchemas{2}(\fCyNodeVar)\quad
      \fDbEdgeType[{\fDbGNames,\fDbEdgeSchema}]?=\fDbRSchemas{2}(\fCyEdgeVar)\\
      \fDbNodeSchema',\fDbEdgeSchema'=\{(\fDbNodeSchemaElem,\fDbEdgeSchemaElem)\in(\fDbNodeSchema\times\fDbEdgeSchema)\mid
        \fDbNodeSchemaElem=\fElemAccess{3}{\fDbEdgeSchemaElem}\lor
        \fDbNodeSchemaElem=\fElemAccess{4}{\fDbEdgeSchemaElem}\}\\
      \fDbNodeSchema'\neq\varnothing\;\land\;\fDbEdgeSchema'\neq\varnothing
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}
                   \fCyEdgeNone{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 }
                 {\fDbRSchemas{2}[
                     {\fCyNodeVar \mapsto \fDbNodeType[{\fDbGNames,\fDbNodeSchema'}]?},
                     {\fCyEdgeVar \mapsto \fDbEdgeType[{\fDbGNames,\fDbEdgeSchema'}]?}
                   ]
                 }
    }
    \and
    \infer[\RuleNameFont\FTyPPatClosedUDirFail]
    {
      \fDbGNames \in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      ?\fDbNodeType = \fDbRSchemas{2}(\fCyNodeVar)\;\lor\;
      ?\fDbEdgeType = \fDbRSchemas{2}(\fCyEdgeVar)
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}
                   \fCyEdgeNone{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 }
                 {\fDbRSchemas{2}[
                     \fCyNodeVar \mapsto ?\fDbNodeType,
                     \fCyEdgeVar \mapsto ?\fDbEdgeType
                 ]}
    }
    \and
    \infer[\RuleNameFont\FTyPPatOpenUDir]
    {
      \fDbGNames \not\in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      ?\fDbNodeType \neq \fDbRSchemas{2}(\fCyNodeVar)\\
      ?\fDbEdgeType \neq \fDbRSchemas{2}(\fCyEdgeVar)
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}
                   \fCyEdgeNone{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 }
                 {\fDbRSchemas{2}}
    }
    \and
    \infer[\RuleNameFont\FTyPPatOpenUDirNull]
    {
      \fDbGNames \not\in \fDom{\fDbSchema}\quad
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {\fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}}
                 {\fDbRSchemas{1}}\quad
      \fPatJudge{\fDbWorld;\fDbRSchemas{1}}
                 {\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 {\fDbRSchemas{2}}\\\\
      ?\fDbNodeType = \fDbRSchemas{2}(\fCyNodeVar)\;\lor\;
      ?\fDbEdgeType = \fDbRSchemas{2}(\fCyEdgeVar)
    }
    {
      \fPatJudge{\fDbWorld;\fDbRSchema}
                 {
                   \fCyElemNodePattern{\fCyNodeVar\,\fPGNodelabel[1]\,\fPGProp[1]}
                   \fCyEdgeNone{\fCyElemEdgePattern{\fCyEdgeVar\,\fPGNodelabel[2]\,\fPGProp[2]}}
                 }
                 {\fDbRSchemas{2}[
                     \fCyNodeVar \mapsto ?\fDbNodeType,
                     \fCyEdgeVar \mapsto ?\fDbEdgeType
                 ]}
    }
\end{mathpar}


==> formalizations/gql-query-typing.tex <==
\begin{mathpar}
  \infer[\RuleNameFont\FTyProjAs]
  {
    \fExpJudgeParam[\fDbWorld;\fDbRSchema;\varnothing]
                   [\fCyExp][\fSortVar][1][\fGroupRef][\fDbVarUse]\\
    \fCyVar \not\in \fDom{\fDbRSchema}
  }
  {
    \fProjJudge{\fDbWorld;\fDbRSchema}
               {\fCyExp\;\fAs\;\fCyVar}
               {\fDbRSchema[\fCyVar \mapsto \fSortVar]}
  }
  \and
  \infer[\RuleNameFont\FTyProj]
  {
    \fProjJudge{\fDbWorld;\fDbRSchema}
               {\fCyExp\;\fAs\;\textbf{\textsf{name}}(\fCyExp)\footnotemark[2]}
               {\fDbRSchemas{1}}               
  }
  {
    \fProjJudge{\fDbWorld;\fDbRSchema}
               {\fCyExp}
               {\fDbRSchemas{1}}
  }
  \and
  \infer[\RuleNameFont\FTyProjList]
  {        
    \fProjJudge{\fDbWorld;\fDbRSchema}
               {\fCyProjection}
               {\fDbRSchemas{1}}\\
    \fProjJudge{\fDbWorld;\fDbRSchema}
               {\fCyExp}
               {\fDbRSchemas{2}}\\\\
    \fDom{\fDbRSchemas{1}}\setminus\fDom{\fDbRSchemas{2}}\neq\varnothing\\
    \fCompatJ{\fDbRSchemas{1}}{\fDbRSchemas{2}}
  }
  {
    \fProjJudge{\fDbWorld;\fDbRSchema}
               {\fCyProjection,\fCyExp}
               {\fSchemaJoin{\fDbRSchemas{1}}{\fDbRSchemas{2}}}
  }
  \and
  \infer[\RuleNameFont\FTyMatchWhereRet]
  {
    \fDbGNames\in\fDom{\fDbCatalog}\quad      
    \fPatExpJudge{\fDbWorld}
                 {\fCyPatternExp}
                 {\fDbRSchemas{1}}\quad
    \fExpJudgeParam[\fDbWorld;\fDbRSchemas{1}]
                   [\fCyPred][\fBool?][1][\fSingletonRef][\fDbVarUse]\quad
    \fProjJudge{\fDbWorld;\fDbRSchemas{1}}
               {\fCyProjection}
               {\fDbRSchemas{2}}
  }
  {
    \fQueryJudge{\fDbWorldS}{\fUse\;\fDbGNames\;\fMatch\;\fCyPatternExp\;\fWhere\;\fCyPred\;\fReturn\;\fCyProjection}{\fDbRSchemas{2}}
  }
  \quad
  \infer[\RuleNameFont\FTyMatchRet]
  {
    \fQueryJudge{\fDbWorldS}{\fUse\;\fDbGNames\;\fMatch\;\fCyPatternExp\;\fWhere\;\fTrue\;\fReturn\;\fCyProjection}{\fDbRSchema}
  }
  {
    \fQueryJudge{\fDbWorldS}{\fUse\;\fDbGNames\;\fMatch\;\fCyPatternExp\;\fReturn\;\fCyProjection}{\fDbRSchema}
  }
  \and
  \infer[\RuleNameFont\FTyCompQueryLift]
  {
    \fQueryJudge{\fDbWorldS}{\fCyQuery}{\fDbRSchema}\\
  }
  {
    \fCompQueryJudge{\fDbWorldS}{\fCyQuery}{\fDbRSchema}
  }
  \and
  \infer[\RuleNameFont\FTyCompQuery]
  {
    \fCompQueryJudge{\fDbWorldS}{\fCyQueryExp}{\fDbRSchemas{1}}\\
    \fQueryJudge{\fDbWorldS}{\fCyQuery}{\fDbRSchemas{2}}\\
    \fCompatC{\fDbRSchemas{1}}{\fDbRSchemas{2}}
  }
  {
    \fCompQueryJudge{\fDbWorldS}{\fCyQueryExp\;\fCyCompOp\;\fCyQuery}{\fDbRSchemas{1}\,\fCyCompOp\,\fDbRSchemas{2}}
  }
\end{mathpar}

